Corrupted Learning Dynamics in Games

Learning in games refers to scenarios where multiple players interact in a shared environment, each aiming to minimize their regret. An equilibrium can be computed at a fast rate of $O(1/T)$ when all players follow the optimistic follow-the-regularized-leader (OFTRL). However, this acceleration is limited to the honest regime, in which all players adhere to a prescribed algorithm -- a situation that may not be realistic in practice. To address this issue, we present corrupted learning dynamics that adaptively find an equilibrium at a rate that depends on the extent to which each player deviates from the strategy suggested by the prescribed algorithm. First, in two-player zero-sum corrupted games, we provide learning dynamics for which the external regret of $x$-player (and similarly for $y$-player) is roughly bounded by $O(\log (m_x m_y) + \sqrt{\hat{C}_y} + \hat{C}_x)$, where $m_x$ and $m_y$ denote the number of actions of $x$- and $y$-players, respectively, and $\hat{C}_x$ and $\hat{C}_y$ represent their cumulative deviations. We then extend our approach to multi-player general-sum corrupted games, providing learning dynamics for which the swap regret of player $i$ is bounded by $O(\log T + \sqrt{\sum_{k} \hat{C}_k \log T} + \hat{C}_i)$ ignoring dependence on the number of players and actions, where $\hat{C}_i$ is the cumulative deviation of player $i$ from the prescribed algorithm. Our learning dynamics are agnostic to the levels of corruption. A key technical contribution is a new analysis that ensures the stability of a Markov chain under a new adaptive learning rate, thereby allowing us to achieve the desired bound in the corrupted regime while matching the best existing bound in the honest regime. Notably, our framework can be extended to address not only corruption in strategies but also corruption in the observed expected utilities, and we provide several matching lower bounds.

==> tex_src_arxiv/7_conclusion.tex <==
\section{Conclusion and future work}
本論文では honest regime と adversarial regime を補間する corrupted regime を考案し，各プレイヤーの与えられたアルゴリズムの出力からの逸脱した度合いに適応的な速度で均衡解を発見する，corrupted learning dynamics を考案した．
我々の two-player zero-sum games と multi-player general-sum games において，既存の最も $T$ への依存性が良いリグレット上界と同等の external or swap regret upper bounds を達成しつつ，corrupted regime においても良好な性能を達成する．
これは optimistic FTRL with adaptive learning rate を用いて実現された．
この性質を活用して scale-free な learning dynamics を簡単に実現可能であることを示した．

多くの面白い future work がある：
\begin{itemize}
  \item adpative learning rate の性質を活用した解析: delayed feedback, ... ? 他の AdaGrad type を持つアルゴリズム
  \item 他の設定における corrupted regime の導入．例えば，
  \begin{itemize}
    \item  last-iterate convergence を持つアルゴリズムでも可能か \citep{wei21linear}
    \item プレイヤー数 $n$ への依存性を改善した no-swap-regret dynamics に対しての利用~\citep{dagan24from,peng24fast}
    \item $\Phi$-regret minimization~\citep{greenwald03general,stoltz07learning,bai22efficient,anagnostides23near}
    \item 他の Nash equilibrium と correlated equilibrium 以外の均衡を得るアルゴリズムへの利用~\citep{fujii23bayes}
    \item partial information setup: semi-bandit feedback~\citep{wei18more} and bandit feedback (cite)
  \end{itemize}
\end{itemize}


% Additional survey:
% \begin{itemize}
%   \item adaptive learning rate (for noisy feedback): \citet{hsieh22noregret}
%   \item care $n$ dependence in swap regret minimization: \citet{dagan24from,peng24fast} and several advances \citet{fujii23bayes}
%   \item $\Phi$-regret minimization: \citet{bai22efficient,anagnostides23near}
% \end{itemize}


